RowHammer: A Retrospective

This retrospective paper describes the RowHammer problem in Dynamic Random Access Memory (DRAM), which was initially introduced by Kim et al. at the ISCA 2014 conference~\cite{rowhammer-isca2014}. RowHammer is a prime (and perhaps the first) example of how a circuit-level failure mechanism can cause a practical and widespread system security vulnerability. It is the phenomenon that repeatedly accessing a row in a modern DRAM chip causes bit flips in physically-adjacent rows at consistently predictable bit locations. RowHammer is caused by a hardware failure mechanism called {\em DRAM disturbance errors}, which is a manifestation of circuit-level cell-to-cell interference in a scaled memory technology. Researchers from Google Project Zero demonstrated in 2015 that this hardware failure mechanism can be effectively exploited by user-level programs to gain kernel privileges on real systems. Many other follow-up works demonstrated other practical attacks exploiting RowHammer. In this article, we comprehensively survey the scientific literature on RowHammer-based attacks as well as mitigation techniques to prevent RowHammer. We also discuss what other related vulnerabilities may be lurking in DRAM and other types of memories, e.g., NAND flash memory or Phase Change Memory, that can potentially threaten the foundations of secure systems, as the memory technologies scale to higher densities. We conclude by describing and advocating a principled approach to memory reliability and security research that can enable us to better anticipate and prevent such vulnerabilities.

==> background.tex <==
\section{Background} 

\label{sec:background}

In this section, we provide the necessary background on DRAM
organization and operation to understand the cause and symptoms of
disturbance errors. 

%For more detail, we refer the reader to prior
%works~\cite{dram-circuit-design, kim12, lee13, liu13}.

\subsection{High-Level Organization}
\label{subsec:high-level}

DRAM chips are manufactured in a variety of
configurations~\cite{jedec-ddr3}, currently ranging in capacities of
1--8~Gbit and in data-bus widths of 4--16~pins. (A particular capacity
does not imply a particular data-bus width.) By itself, an individual
DRAM chip has only a small capacity and a narrow data-bus. That is why
multiple DRAM chips are commonly ganged together to provide a large
capacity and a wide data-bus (typically 64-bit). Such a ``gang'' of DRAM
chips is referred to as a DRAM {\em rank}. One or more ranks are
soldered onto a circuit board to form a DRAM {\em module}.


\subsection{Low-Level Organization}
\label{subsec:low-level}

As Figure~\ref{fig:cella} shows, DRAM comprises a two-dimensional array of
DRAM {\em cells}, each of which consists of a {\em capacitor} and an
{\em access-transistor}. Depending on whether its capacitor is fully
charged or fully discharged, a cell is in either the {\em charged state}
or the {\em discharged state}, respectively. These two states are used
to represent a binary data value.

\input{cell}

%Better known as {\em sense-amplifiers}, the function of the row-buffer
%is to detect whether charge exists in the cells and to strengthen them
%by driving the bitline voltage to either high or
%low~\cite{dram-circuit-design, kim12, lee13}. 

As Figure~\ref{fig:cellb} shows, every cell lies at the intersection of
two perpendicular wires: a horizontal {\em wordline} and a vertical {\em
bitline}. A wordline connects to all cells in the horizontal direction
({\em row}) and a bitline connects to all cells in the vertical
direction ({\em column}). When a row's wordline is {\em raised} to a
high voltage, it enables all of the access-transistors within the row,
which in turn connects all of the capacitors to their respective
bitlines. This allows the row's data (in the form of charge) to be
transferred into the {\em row-buffer} shown in Figure~\ref{fig:cella}.
Better known as {\em sense-amplifiers}, the row-buffer reads out the
charge from the cells --- a process that destroys the data in the cells
--- and immediately writes the charge back into the
cells~\cite{dram-circuit-design, kim12, lee13}. Subsequently, all
accesses to the row are served by the row-buffer on behalf of the row.
When there are no more accesses to the row, the wordline is {\em
lowered} to a low voltage, disconnecting the capacitors from the
bitlines. A group of rows is called a {\em bank}, each of which has its
own dedicated row-buffer. (The organization of a bank is similar to what
was shown in Figure~\ref{fig:cella}.) Finally, multiple banks come
together to form a rank. For example, Figure~\ref{fig:mctrl} shows a 2GB
rank whose 256K rows are vertically partitioned into eight banks of 32K
rows, where each row is 8KB ($=$64Kb) in size~\cite{jedec-ddr3}. Having
multiple banks increases parallelism because accesses to different banks
can be served concurrently. 

%\vspace{-1ex}
\input{mctrl}


\subsection{Accessing DRAM} 
\label{subsec:accessing}

An access to a rank occurs in three steps: {\em (i)}~``opening'' the
desired row within a desired bank, {\em (ii)}~accessing the desired
columns from the row-buffer, and {\em (iii)}~``closing'' the row. 

\begin{enumerate}[leftmargin=1.3em]

\item Open Row. A row is opened by raising its wordline. This connects
the row to the bitlines, transferring all of its data into the bank's
row-buffer.

\item Read/Write Columns. The row-buffer's data is accessed by reading
or writing any of its columns as needed.

\item Close Row. Before a different row in the same bank can be opened,
the original row must be closed by lowering its wordline. In addition,
the row-buffer is cleared.

\end{enumerate}

The {\em memory controller}, which typically resides in the processor
(Figure~\ref{fig:mctrl}), guides the rank through the three steps by
issuing {\em commands} and {\em addresses} as summarized in
Table~\ref{tab:commands}. After a rank accepts a command, some amount of
delay is required before it becomes ready to accept another command.
This delay is referred to as a DRAM {\em timing
constraint}~\cite{jedec-ddr3}. For example, the timing constraint
defined between a pair of {\tt ACTIVATEs} to the same row (in the same
bank) is referred to as \trc (row cycle time), whose typical value is
$\sim$50~{\em nanoseconds}~\cite{jedec-ddr3}. When trying to open and
close the same row as quickly as possible, \trc becomes the bottleneck
--- limiting the maximum rate to once every \trc.

\input{commands}



\subsection{Refreshing DRAM}
\label{subsec:refreshing}

The charge stored in a DRAM cell is not persistent. This is due to
various leakage mechanisms by which charge can disperse: e.g.,
subthreshold leakage \cite{roy03} and gate-induced drain
leakage~\cite{saino00}. Eventually, the cell's charge-level would
deviate beyond the noise margin, causing it to lose data --- in other
words, a cell has only a limited {\em retention time}. Before this time
expires, the cell's charge must be restored (i.e., {\em refreshed}) to
its original value: fully charged or fully discharged. The DDR3 DRAM
specifications~\cite{jedec-ddr3} guarantee a retention time of at least
64 {\em milliseconds}, meaning that all cells within a rank need to be
refreshed at least once during this time window. Refreshing a cell can
be accomplished by opening the row to which the cell belongs. Not only
does the row-buffer read the cell's altered charge value but, at the
same time, it restores the charge to full value
(Section~\ref{subsec:low-level}). In fact, {\em refreshing a row and
opening a row are identical operations} from a circuits perspective.
Therefore, one possible way for the memory controller to refresh a rank
is to issue an \cmda command to every row in succession. In practice,
there exists a separate \cmdf command which refreshes many rows at a
time (Table~\ref{tab:commands}). When a rank receives a \cmdf, it
automatically refreshes several of its least-recently-refreshed rows by
internally generating \cmda and \cmdp pairs to them. Within any given
64{\em ms} time window, the memory controller issues a sufficient number
of \cmdf commands to ensure that every row is refreshed exactly once.
For a DDR3 DRAM rank, the memory controller issues 8192 \cmdf commands
during 64{\em ms}, once every 7.8{\em us} ($=$64{\em
ms}/8192)~\cite{jedec-ddr3}.




==> cell.tex <==

\begin{figure}[h]
\centering
\begin{subfigure}[b]{0.45\linewidth}
\centering
\includegraphics[height=1.1in]{micro_cella}
\subcaption{Rows of cells}
\label{fig:cella}
\end{subfigure}
\hspace{0.00in}
\begin{subfigure}[b]{0.45\linewidth}
\centering
\includegraphics[height=1.1in]{micro_cellb}
\subcaption{A single cell}
\label{fig:cellb}
\end{subfigure}

\caption{DRAM consists of cells}
\label{fig:cell}
\end{figure}

%\subfigure[Physical Organization]{
%\label{fig:ranka}
%\includegraphics[height=1.05in]{figures/micro_ranka}
%}
%\subfigure[Logical Abstraction]{
%\label{fig:rankb}
%\includegraphics[height=1.05in]{figures/micro_rankb}
%}


==> commands.tex <==

\begin{table}[h]
\centering
\small
%\footnotesize
\begin{tabular}{lll}
\toprule
{\em Operation}                             & {\em Command}     & {\em Address(es)} \\
\midrule
1. Open Row                                 & {\tt ACTIVATE} {\tt (ACT)}              & Bank, Row       \\
%\cmidrule(lr){1-3}
2. Read/Write Column                        & \cmdr/\cmdw                   & Bank, Column    \\
%\cmidrule(lr){1-3}
3. Close Row                                & {\tt PRECHARGE} {\tt (PRE)}             & Bank              \\
\cmidrule(lr){1-3}
%\midrule
Refresh (Section~\ref{subsec:refreshing})   & {\tt REFRESH} {\tt (REF)}               & ---               \\
\bottomrule
\end{tabular}
\caption{DRAM commands and addresses~\cite{jedec-ddr3}} 
\label{tab:commands}
\end{table}



==> mctrl.tex <==
\begin{figure}[h]
\centering
\includegraphics[width=0.90\linewidth]{micro_mctrl}
\caption{Memory controller, buses, rank, and banks}
\label{fig:mctrl}
\end{figure}


